Formal Explanations for Neuro-Symbolic AI

Despite the practical success of Artificial Intelligence (AI), current neural AI algorithms face two significant issues. First, the decisions made by neural architectures are often prone to bias and brittleness. Second, when a chain of reasoning is required, neural systems often perform poorly. Neuro-symbolic artificial intelligence is a promising approach that tackles these (and other) weaknesses by combining the power of neural perception and symbolic reasoning. Meanwhile, the success of AI has made it critical to understand its behaviour, leading to the development of explainable artificial intelligence (XAI). While neuro-symbolic AI systems have important advantages over purely neural AI, we still need to explain their actions, which are obscured by the interactions of the neural and symbolic components. To address the issue, this paper proposes a formal approach to explaining the decisions of neuro-symbolic systems. The approach hinges on the use of formal abductive explanations and on solving the neuro-symbolic explainability problem hierarchically. Namely, it first computes a formal explanation for the symbolic component of the system, which serves to identify a subset of the individual parts of neural information that needs to be explained. This is followed by explaining only those individual neural inputs, independently of each other, which facilitates succinctness of hierarchical formal explanations and helps to increase the overall performance of the approach. Experimental results for a few complex reasoning tasks demonstrate practical efficiency of the proposed approach, in comparison to purely neural systems, from the perspective of explanation size, explanation time, training time, model sizes, and the quality of explanations reported.

==> rebuttal.tex <==
\input{_preamble.tex}
\input{rebuttal_img_tables.tex}
\input{_postamble.tex}


==> rebuttal_img_tables.tex <==
\section{Additional Results: Scallop-SHAP} \label{sec:res}

\begin{figure}[th]
  %
  \centering
  %
  \begin{subfigure}[b]{0.35\textwidth}
    %
    \includegraphics[width=\textwidth]{lex8T}
    %
    \caption{Positive example}
    %
    \label{fig:lex8T}
    %
  \end{subfigure}%
  %
  \hfill
  %
  \begin{subfigure}[b]{0.35\textwidth}
    %
    \includegraphics[width=\textwidth]{lex8F}
    %
    \caption{Negative example}
    %
    \label{fig:lex8F}
    %
    \end{subfigure}
  %
  \caption{[extending Figure $4$ of paper]. Query: The top row 4-digit binary number is greater than the bottom row 4-digit binary number. Answer: True or False.}
  %
\label{fig:lex8}
  %
\end{figure}

\begin{figure}[th]
  %
  \centering
  %
  \begin{subfigure}[b]{0.35\textwidth}
    %
    \includegraphics[width=\textwidth]{rg10T}
    %
    \caption{Positive example}
    %
    \label{fig:rg10T}
    %
  \end{subfigure}%
  %
  \hfill
  %
  \begin{subfigure}[b]{0.35\textwidth}
    %
    \includegraphics[width=\textwidth]{rg10F}
    %
    \caption{Negative example}
    %
    \label{fig:rg10F}
    %
    \end{subfigure}
  %
  \caption{[extending Figure $5$ of paper]. Query: This binary string is a member of the regular language $R_2$. Answer: True or False.}
  %
\label{fig:regex10}
  %
\end{figure}

%
\begin{figure}[th]
  %
  \centering
  %
  \begin{subfigure}[b]{0.20\textwidth}
    %
    \includegraphics[width=\textwidth]{p4}
    %
    \caption{\texttt{HX-Marabou-e<1}}
    %
    \label{fig:p4}
    %
  \end{subfigure}
  %
  \hfill
  %
  \begin{subfigure}[b]{0.20\textwidth}
    %
    \includegraphics[width=\textwidth]{p5}
    %
    \caption{\texttt{HX-SHAP}}
    %
    \label{fig:p5}
    %
  \end{subfigure}
  %
  \hfill
  %
  \begin{subfigure}[b]{0.20\textwidth}
    %
    \includegraphics[width=\textwidth]{p6}
    %
    \caption{\texttt{NN-SHAP}}
    %
    \label{fig:p6}
    %
  \end{subfigure}
  %
  \hfill
  %
  \begin{subfigure}[b]{0.20\textwidth}
    %
    \includegraphics[width=\textwidth]{p7}
    %
    \caption{\texttt{Scallop-SHAP}}
    %
    \label{fig:p7}
    %
  \end{subfigure}
  %
  \hfill
  %
  \caption{[extending Figure $6$ of paper]. Query: What is the length of the shortest path? Answer: 5.}
  %
\label{fig:pac}
  %
\end{figure}
%
\begin{table}[h!]
  \setlength{\tabcolsep}{3pt}
  %
  \caption{\label{tab:expl} Explanation size statistics for each evaluated explanation methods and benchmarks. Each column min, avg, max, and time depict the minimum, average, and maximum size of explanation, and average explanation computation time (MM:SS or HH:MM:SS) respectively.}
  % \begin{adjustbox}{center}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrrr@{}}
    %
    \toprule
    & \multicolumn{4}{c}{ \texttt{HX-Marabou-e=1} } & \multicolumn{4}{c}{ \texttt{HX-Marabou-e<1} } & \multicolumn{4}{c}{ \texttt{HX-SHAP} } & \multicolumn{4}{c}{ \texttt{NN-SHAP} } & \multicolumn{4}{c}{ \texttt{Scallop-SHAP} } \\
    %
    \cmidrule(l){2-5}\cmidrule(l){6-9}\cmidrule(l){10-13}\cmidrule(l){14-17}\cmidrule(l){18-21}
    %
    Benchmark & min & avg & max & time & min & avg & max & time & min & avg & max & time & min & avg & max & time & min & avg & max & time \\
    \midrule
    %
    Lex1-6 & 746 & 1087 & 1768 & 02:04 & 298 & 552 & 919 & 01:54 & 781 & 1108 & 1764 & 00:01 & 2641 & 2687 & 2753 & 00:07 & 138 & 430 & 488 & 08:55\\
    %
    Lex1-8 & 733 & 1126 & 2155 & 02:25 & 302 & 605 & 1201 & 02:10 & 1008 & 1414 & 2645 & 00:01 & 3480 & 3558 & 3612 & 00:04 & 316 & 459 & 498 & 21:25\\
    %
    RegExp-1-6 & 326 & 571 & 1854 & 00:50 & 70 & 328 & 1185 & 00:48 & 470 & 705 & 2029 & 00:01 & 2616 & 2679 & 2742 & 00:08 & 233 & 406 & 492 & 08:31\\
    %
    RegExp-1-8 & 499 & 771 & 2357 & 00:53 & 305 & 562 & 1808 & 01:10 & 501 & 690 & 2068 & 00:01 & 3486 & 3550 & 3626 & 00:08 & 297 & 435 & 490 & 16:37\\
    %
    RegExp2-10 & 832 & 1422 & 2778 & 02:42 & 296 & 742 & 1522 & 02:18 & 972 & 1570 & 3126 & 00:01 & 4408 & 4474 & 4579 & 00:10 & 191 & 435 & 498 & 25:53\\
    %
    Pacman-SP & 721 & 1617 & 2902 & 08:13 & 398 & 1033 & 1784 & 10:04 & 800 & 1728 & 3200 & 00:01 & 6957 & 7038 & 7040 & 05:14 & 391 & 456 & 522 & 20:39:18\\
    %
    \bottomrule
    %
  \end{tabular}
  % \end{adjustbox}
}
\end{table}

